Optimal Linear Decay Learning Rate Schedules and Further Refinements

Learning rate schedules used in practice bear little resemblance to those recommended by theory. We close much of this theory/practice gap, and as a consequence are able to derive new problem-adaptive learning rate schedules. Our main technical contribution is a refined analysis of learning rate schedules for a wide class of optimization algorithms (including SGD). When considering only worst-case analysis, our theory predicts that the optimal choice is the linear decay schedule where the step-size is set proportional to 1 - t/T, where t is the current iteration and T is the total number of steps. To go beyond this worst-case analysis, we use the observed gradient norms to derive schedules refined for any particular task. These refined schedules exhibit learning rate warm-up and rapid learning rate annealing near the end of training. Ours is the first systematic approach to automatically yield both of these properties. We perform the most comprehensive evaluation of learning rate schedules to date, evaluating across 10 diverse deep learning problems, a series of LLMs, and a suite of logistic regression problems. We validate that overall, the linear-decay schedule outperforms all commonly used default schedules including cosine annealing. Our adaptive schedule refinement method gives further improvements.

==> scratch.tex <==
\section{All-Tail Summation Bound}\label{sec:proof:tail}

\subsection{Existing bound}
\begin{lemma}
Let $q_{t}\geq0$, and let $\eta_{t}$ be a positive non-increasing
sequence. Then:
% \[
% \eta_{T}q_{T}\leq\frac{1}{T}\sum_{t=1}^{T}\eta_{t}q_{t}+\sum_{k=1}^{T-1}\frac{1}{k(k+1)}\sum_{t=T-k+1}^{T}\eta_{t}\left(q_{t}-q_{T-k}\right)
% \]
\[
\eta_{T}q_{T}\leq\frac{1}{T}\sum_{t=1}^{T}\eta_{t}q_{t}+\sum_{k=1}^{T-1}\frac{1}{k(k+1)}\sum_{t=k+1}^{T}\eta_{t}\left(q_{t}-q_{k}\right),
\]
\end{lemma}

\begin{proof}
We present below a version of his proof that's written to move the
single inequality application in the whole proof to the last step.
Define $S_{k}=\frac{1}{k}\sum_{t=T-k+1}^{T}\eta_{t}q_{t}$.

Then
\begin{align*}
kS_{k} & =(k+1)S_{k+1}-\eta_{T-k}q_{T-k}\\
 & =ks_{k+1}+S_{k+1}-\eta_{T-k}q_{T-k}\\
 & =ks_{k+1}+\frac{1}{k+1}\sum_{t=T-k}^{T}\left(\eta_{t}q_{t}-\eta_{T-k}q_{T-k}\right)
\end{align*}

Dividing through by $k$:
\[
S_{k}=S_{k+1}+\frac{1}{k(k+1)}\sum_{t=T-k}^{T}\left(\eta_{t}q_{t}-\eta_{T-k}q_{T-k}\right)
\]

Unrolling, we have:
\[
S_{1}=S_{T}+\sum_{k=1}^{T-1}\frac{1}{k(k+1)}\sum_{t=T-k}^{T}\left(\eta_{t}q_{t}-\eta_{T-k}q_{T-k}\right).
\]

Now we use $S_{1}=\eta_{T}q_{T}$. Note that the first entry in that
sum is zero so we may shift the indexing to start at $t=T-k+1$. Giving:
\begin{align*}
\eta_{T}q_{T} & =S_{T}+\sum_{k=1}^{T-1}\frac{1}{k(k+1)}\sum_{t=T-k+1}^{T}\left(\eta_{t}q_{t}-\eta_{T-k}q_{T-k}\right)\\
 & \leq S_{T}+\sum_{k=1}^{T-1}\frac{1}{k(k+1)}\sum_{t=T-k+1}^{T}\eta_{t}\left(q_{t}-q_{T-k}\right).
\end{align*}

Where the final step uses the fact that $\eta_{t}$ is decreasing.
Plugging in the definition of $S_{T}$, and substituting $k=T-k$ to simplify gives the result.
\end{proof}

\subsection{Improved Expression}
\begin{lemma}\label{lem:tail}
Let $q_{t}$ be any sequence, and let $\eta_{t}$ be a positive sequence.
Then:
% \[
% q_{T}=\frac{1}{\sum_{t=1}^{T}\eta_{t}}\sum_{t=1}^{T}\eta_{t}q_{t}+\sum_{k=1}^{T-1}\frac{\eta_{T-k}}{\sum_{t=T-k+1}^{T}\eta_{t}}\left(\frac{1}{\sum_{t=T-k}^{T}\eta_{t}}\sum_{t=T-k}^{T}\eta_{t}\left(q_{t}-q_{T-k}\right)\right)
% \]
\begin{align*}
q_{T}&=\frac{1}{\sum_{t=1}^{T}\eta_{t}}\sum_{t=1}^{T}\eta_{t}q_{t}+\sum_{k=1}^{T-1}\frac{\eta_{k}}{\sum_{t=k+1}^{T}\eta_{t}}\left(\frac{1}{\sum_{t=k}^{T}\eta_{t}}\sum_{t=k}^{T}\eta_{t}\left(q_{t}-q_{k}\right)\right)\\
&=\frac{1}{\w_{1:T}}\sum_{t=1}^{T}\w_{t}q_{t}+\sum_{k=1}^{T-1}\left(\frac{1}{\w_{k+1:T}} - \frac{1}{\w_{k:T}}\right)\sum_{t=k}^{T}\w_{t}\left(q_{t}-q_{k}\right).
\end{align*}
\end{lemma}

\begin{proof}
Define
\[
S_{k}=\frac{1}{\sum_{t=T-k+1}^{T}\eta_{t}}\sum_{t=T-k+1}^{T}\eta_{t}q_{t}.
\]
Note that with this definition:
\[
S_{1}=\frac{1}{\sum_{t=T}^{T}\eta_{t}}\sum_{t=T}^{T}\eta_{t}q_{t}=q_{T},
\]
and $S_{T}$ is the full sum:
\[
S_{T}=\frac{1}{\sum_{t=1}^{T}\eta_{t}}\sum_{t=1}^{T}\eta_{t}q_{t}.
\]
The difference from the weighting used in the the Lemma above: we
normalized by the sum of the step sizes rather than $k$. We get the
following expansion: 

\begin{align*}
\left(\sum_{t=T-k+1}^{T}\eta_{t}\right)S_{k} & =\sum_{t=T-k+1}^{T}\eta_{t}q_{t}\\
 & =\sum_{t=T-k}^{T}\eta_{t}q_{t}-\eta_{T-k}q_{T-k}\\
 & =\left(\sum_{t=T-k}^{T}\eta_{t}\right)S_{k+1}-\eta_{T-k}q_{T-k}\\
 & =\left(\sum_{t=T-k+1}^{T}\eta_{t}\right)S_{k+1}+\left(\eta_{T-k}S_{k+1}-\eta_{T-k}q_{T-k}\right)
\end{align*}
So dividing through by $\sum_{t=T-k+1}^{T}\eta_{t}$:
\[
S_{k}=S_{k+1}+\frac{\eta_{T-k}}{\sum_{t=T-k+1}^{T}\eta_{t}}\left(S_{k+1}-q_{T-k}\right)
\]
Unrolling
\[
S_{1}=S_{T}+\sum_{k=1}^{T-1}\frac{\eta_{T-k}}{\sum_{t=T-k+1}^{T}\eta_{t}}\left(S_{k+1}-q_{T-k}\right)
\]
Note that, plugging in $S_{k+1}$:

\begin{align*}
S_{k+1}-q_{T-k} & =\frac{1}{\sum_{t=T-k}^{T}\eta_{t}}\sum_{t=T-k}^{T}\eta_{t}q_{t}-q_{T-k}\\
 & =\frac{1}{\sum_{t=T-k}^{T}\eta_{t}}\sum_{t=T-k}^{T}\eta_{t}\left(q_{t}-q_{T-k}\right)
\end{align*}
So we have:
\[
q_{T}=\frac{1}{\sum_{t=1}^{T}\eta_{t}}\sum_{t=1}^{T}\eta_{t}q_{t}+\sum_{k=1}^{T-1}\frac{\eta_{T-k}}{\sum_{t=T-k+1}^{T}\eta_{t}}\left(\frac{1}{\sum_{t=T-k}^{T}\eta_{t}}\sum_{t=T-k}^{T}\eta_{t}\left(q_{t}-q_{T-k}\right)\right).
\]
Substituting $k=T-k$ to simplify gives the result.
\end{proof}
\begin{remark}
By using a weighting sequence $\eta_{t}$ elsewhere, we are able to
remove the $\eta_{T}$ weight from in front of the $q_{T}$ term.
This is crucial as we want to be able to analyze schedules where the
learning rate drops extremely small near the end of optimization,
and yet still bound $q_{T}=f(x_{T})-f_{*}$, but if $q_{T}$ is weighted
by $\eta_{T}$ we will get very loose bounds when $\eta_{T}$ is small.
Notice also that we have an equality instead of an inequality, and
we have not had to impose the requirement that $\eta$ be a non-increasing
sequence.
\end{remark}


% \begin{restatable}{lemma}{lemtail}\label{lem:tail}
% Let $q_{t}$ be any sequence, and let $\w_{t}$ be a positive sequence.
% Then:
% \begin{align*}
% q_{T}&=\frac{1}{\sum_{t=1}^{T}\w_{t}}\sum_{t=1}^{T}\w_{t}q_{t}+\sum_{k=1}^{T-1}\frac{\w_{T-k}}{\sum_{t=T-k+1}^{T}\w_{t}}\left(\frac{1}{\sum_{t=T-k}^{T}\w_{t}}\sum_{t=T-k}^{T}\w_{t}\left(q_{t}-q_{T-k}\right)\right)\\
% &=\frac{1}{\w_{1:T}}\sum_{t=1}^{T}\w_{t}q_{t}+\sum_{k=1}^{T-1}\left(\frac{1}{\w_{T-k+1:T}} - \frac{1}{\w_{T-k:T}}\right)\sum_{t=T-k}^{T}\w_{t}\left(q_{t}-q_{T-k}\right)
% \end{align*}
% \end{restatable}

% \begin{proof}
% Define
% \[
% S_{k}=\frac{1}{\sum_{t=T-k+1}^{T}\w_{t}}\sum_{t=T-k+1}^{T}\w_{t}q_{t}.
% \]
% Note that with this definition:
% \[
% S_{1}=\frac{1}{\sum_{t=T}^{T}\w_{t}}\sum_{t=T}^{T}\w_{t}q_{t}=q_{T},
% \]
% and $S_{T}$ is the full sum:
% \[
% S_{T}=\frac{1}{\sum_{t=1}^{T}\w_{t}}\sum_{t=1}^{T}\w_{t}q_{t}.
% \]
% The difference from the weighting used in the the Lemma above: we
% normalized by the sum of the step sizes rather than $k$. We get the
% following expansion: 

% \begin{align*}
% \left(\sum_{t=T-k+1}^{T}\w_{t}\right)S_{k} & =\sum_{t=T-k+1}^{T}\w_{t}q_{t}\\
%  & =\sum_{t=T-k}^{T}\w_{t}q_{t}-\w_{T-k}q_{T-k}\\
%  & =\left(\sum_{t=T-k}^{T}\w_{t}\right)S_{k+1}-\w_{T-k}q_{T-k}\\
%  & =\left(\sum_{t=T-k+1}^{T}\w_{t}\right)S_{k+1}+\left(\w_{T-k}S_{k+1}-\w_{T-k}q_{T-k}\right)
% \end{align*}
% So dividing through by $\sum_{t=T-k+1}^{T}\w_{t}$:
% \[
% S_{k}=S_{k+1}+\frac{\w_{T-k}}{\sum_{t=T-k+1}^{T}\w_{t}}\left(S_{k+1}-q_{T-k}\right)
% \]
% Unrolling
% \[
% S_{1}=S_{T}+\sum_{k=1}^{T-1}\frac{\w_{T-k}}{\sum_{t=T-k+1}^{T}\w_{t}}\left(S_{k+1}-q_{T-k}\right)
% \]
% Note that, plugging in $S_{k+1}$:

% \begin{align*}
% S_{k+1}-q_{T-k} & =\frac{1}{\sum_{t=T-k}^{T}\w_{t}}\sum_{t=T-k}^{T}\w_{t}q_{t}-q_{T-k}\\
%  & =\frac{1}{\sum_{t=T-k}^{T}\w_{t}}\sum_{t=T-k}^{T}\w_{t}\left(q_{t}-q_{T-k}\right)
% \end{align*}
% So we have:
% \[
% q_{T}=\frac{1}{\sum_{t=1}^{T}\w_{t}}\sum_{t=1}^{T}\w_{t}q_{t}+\sum_{k=1}^{T-1}\frac{\w_{T-k}}{\sum_{t=T-k+1}^{T}\w_{t}}\left(\frac{1}{\sum_{t=T-k}^{T}\w_{t}}\sum_{t=T-k}^{T}\w_{t}\left(q_{t}-q_{T-k}\right)\right).
% \]
% \end{proof}

\section{Proof of Theorem ~\ref{thm:additive}}\label{sec:proof:thmadditive}

Before proving Theorem~\ref{thm:additive}, we need the following important Lemma:

\begin{restatable}{lemma}{lemrearrange}\label{lem:rearrange}
    Suppose $z_1,\dots,z_T$ is an arbitrary sequence of vectors. Let $\w_1,\dots,\w_T$ be an arbitrary sequence of positive numbers. Define the sequence  $x_1,\dots,x_T$ by:
\begin{align*}
    x_t = \w_{t:T}\left( \frac{z_t}{\w_{1:T}} + \sum_{p=1}^{t-1} x_p\left(\frac{1}{\w_{p+1:T}}-\frac{1}{\w_{p:T}}\right)\right)
\end{align*}
Suppose $g_t$ are random variables. with $\E[g_t|x_1,\dots,x_t] \in \partial f(x_t)$ for some convex $f$. Then:
\begin{align*}
\E[f(x_T) - f(u)] &\le \E\left[\frac{1}{\w_{1:T}}\sum_{t=1}^T\w_t\langle g_t, z_t - u\rangle \right]
\end{align*}
\end{restatable}
\begin{proof}
Let us set $q_t = f(x_t) - f(u)$. Then we have $\E[q_t] \le \E[\langle g_t , x_t -u\rangle]$ and $\E[q_t -q_k]\le \E[\langle g_t, x_t - x_k\rangle]$. With this, we have:
\begin{align*}
    \E[q_T]&\le \E\left[\frac{1}{\w_{1:T}} \sum_{t=1}^T \w_t \langle g_t, x_t - u\rangle + \sum_{k=1}^{T-1}\left(\frac{1}{\w_{T-k+1:T}} - \frac{1}{\w_{T-k:T}}\right) \sum_{t=T-k}^T \w_t \langle g_t, x_t - x_{T-k}\rangle \right]
\end{align*}
Now, let us find the coefficient of $\langle g_t, x_t\rangle$ in the above expression. This is:
\begin{align*}
    &\frac{\w_t}{\w_{1:T}} + \sum_{k=T-t}^{T-1} \left(\frac{1}{\w_{T-k+1:T}} - \frac{1}{\w_{T-k:T}}\right) \w_t -\w_t\left(\frac{1}{\w_{t+1:T}} - \frac{1}{\w_{t:T}}\right)\\
    &=\frac{\w_t}{\w_{1:T}} + \sum_{k=T-t+1}^{T-1} \left(\frac{1}{\w_{T-k+1:T}} - \frac{1}{\w_{T-k:T}}\right) \w_t\\
    &=\frac{\w_t}{\w_{t:T}}
\end{align*}
Next, for $p<t$, the coefficient of $\langle g_t, x_p\rangle$ is:
\begin{align*}
    -\left(\frac{1}{\w_{p+1:T}}-\frac{1}{\w_{p:T}}\right)\w_t
\end{align*}
And for $p>t$, the coefficient of $\langle g_t, x_p\rangle$ is zero. Finally the coefficient of $\langle g_t, u\rangle$ is $-\frac{\w_t}{\w_{1:T}}$.

Putting this all together, we can rearrange the expression as follows:
\begin{align*}
    \E[q_T]&\le \E\left[ \sum_{t=1}^T \left\langle g_t, \frac{\w_t}{\w_{t:T}}x_t -\left(\frac{\w_t u}{\w_{1:T}}  +\sum_{p=1}^{t-1} \w_t x_t \left(\frac{1}{\w_{p+1:T}}-\frac{1}{\w_{p:T}}\right) \right)\right\rangle \right]\\
    &= \E\left[ \sum_{t=1}^T\left\langle \frac{\w_t}{\w_{t:T}} g_t, x_t - \w_{t:T}\left( \frac{u}{\w_{1:T}} + \sum_{p=1}^{t-1} x_p\left(\frac{1}{\w_{p+1:T}}-\frac{1}{\w_{p:T}}\right)\right) \right\rangle\right]
\end{align*}

Now, given an arbitrary sequence $z_1,\dots,z_T$, define $x_t$ recursively by:
\begin{align*}
    x_t = \w_{t:T}\left( \frac{z_t}{\w_{1:T}} + \sum_{p=1}^{t-1} x_p\left(\frac{1}{\w_{p+1:T}}-\frac{1}{\w_{p:T}}\right)\right)
\end{align*}
Then we have:
\begin{align*}
    \E[q_T]&\le \E\left[\sum_{t=1}^T\frac{\w_t}{\w_{1:T}} \langle g_t, z_t - u\rangle \right]
\end{align*}
\end{proof}

Now, we are finally ready to prove the Theorem~\ref{thm:additive}:

\thmadditive*

\begin{proof}
Let's define $\hat x_1=z_t$ and recursively set:
\begin{align*}
    \hat x_t = w_{t:T} \left(\frac{z_t}{w_{1:T}} + \sum_{p=1}^{t-1} \hat x_p\left(\frac{1}{w_{p+1:T}} - \frac{1}{w_{p:T}}\right)\right)
\end{align*}
Then, Lemma~\ref{lem:rearrange} shows that $\E[f(x_T) - f(u)] \le \E\left[\frac{1}{\w_{1:T}}\sum_{t=1}^T\w_t\langle g_t, z_t - u\rangle \right]$. So, it suffices to show that $x_t=\hat x_t$ for all $t$. In turn, since $\hat x_1 = z_1=x_1$, it suffices to show $\hat x_{t+1}-\hat x_t = \frac{w_{t+1:T}}{w_{1:T}} \Delta_t=x_{t+1}-x_t$ for all $t$.

To this end, let's do some calculation. First:
\begin{align*}
    \hat x_t &=   \frac{\w_t}{\w_{t:T}}x_t + \frac{\w_{t+1:T}}{\w_{t:T}}x_t\\
    &= \frac{\w_t}{\w_{t:T}} \hat x_t +\w_{t+t:T}\left( \frac{z_t}{\w_{1:T}} + \sum_{p=1}^{t-1} \hat x_p\left(\frac{1}{\w_{p+1:T}}-\frac{1}{\w_{p:T}}\right)\right)
\end{align*}
With this expression, we have:
\begin{align*}
\hat x_{t+1} - \hat x_t &= \hat x_{t+1} - \w_{t+1:T}\left( \frac{z_{t+1}}{\w_{1:T}} + \sum_{p=1}^{t} x_p\left(\frac{1}{\w_{p+1:T}}-\frac{1}{\w_{p:T}}\right)\right)  - \frac{\w_t}{\w_{t:T}} \hat x_t \\
&=w_{t+1:T} \left(\frac{z_{t+1}}{w_{1:T}} + \sum_{p=1}^{t} \hat x_p\left(\frac{1}{w_{p+1:T}} - \frac{1}{w_{p:T}}\right)\right)\\
&\qquad-  \w_{t+1:T}\left( \frac{z_t}{\w_{1:T}} + \sum_{p=1}^{t-1} x_p\left(\frac{1}{\w_{p+1:T}} -\frac{1}{\w_{p:T}}\right)\right) - \frac{\w_t}{\w_{t:T}} \hat x_t \\
&= \frac{\w_{t+1:T} (z_{t+1} -  z_t)}{\w_{1:T}} + \w_{t+1:T} \hat x_t\left(\frac{1}{\w_{t+1:T}} - \frac{1}{\w_{t:T}}\right) - \frac{\w_t}{\w_{t:T}} \hat x_t\\
&= \frac{\w_{t+1:T}}{\w_{1:T}} \Delta_t + \hat x_t\left(1-\frac{\w_{t+1:T} +\w_t}{\w_{t:T}}\right)\\
&= \frac{\w_{t+1:T}}{\w_{1:T}} \Delta_t
\end{align*}
\end{proof}


\section{Proof of Theorem~\ref{thm:optimal}}\label{sec:proof:optimal}

\thmoptimal*

\begin{proof}
    First, observe that with $\Delta_t = -\w_t \eta_t$, we have $x_{t+1} = x_t + \frac{\w_{t+1:T}}{\w_{1:T}} \Delta_t$. Therefore with $z_1=x_1$ and $z_{t+1} = z_t +\Delta_t$, Theorem~\ref{thm:additive} implies:
    \begin{align*}
        \E[f(x_T) - f(\cmp)]&\le \E\left[\frac{1}{\w_{1:T}} \sum_{t=1}^T \langle \w_t g_t,z_t -\cmp\rangle\right]
    \end{align*}
    Next, observe that $z_t$ is simply online gradient descent with learning rate 1 acting on the loss vectors $\w_t z_t$. Standard analysis \citep{zinkevich2003online} shows:
    \begin{align*}
        \sum_{t=1}^T \langle \w_t g_t,z_t -\cmp\rangle& = \frac{\|z_1-\cmp\|^2}{2} - \frac{\|z_{T+1}-\cmp\|^2}{2} +\sum_{t=1}^T \frac{\w_t^2 \|g_t\|^2}{2}
    \end{align*}
    This immediately implies the first part of the Theorem. Next, we need to solve for the minimizing values of $\w_t$. To do this, we take the logarithm of the expression $\frac{1}{2\w_{1:T}}\left(\|x_1-\cmp\|^2 + \sum_{t=1}^T \w_t^2\|g_t\|^2\right)$ and differentiate:
    \begin{align*}
        \frac{\partial}{\partial \w_k} \log\left[\frac{1}{2 \w_{1:T}}\left(\|x_1-\cmp\|^2 + \sum_{t=1}^T \w_t^2\|g_t\|^2\right)\right]&= \frac{2\w_k \|g_k\|^2}{\|x_1-\cmp\|^2 + \sum_{t=1}^T \w_t^2\|g_t\|^2} -\frac{1}{\w_{1:T}}
    \end{align*}
    We set this equal to zero to solve for the optimal $\w_k$:
    \begin{align*}
    \w_k &= \|g_k\|^{-2}\frac{\|x_1-\cmp\|^2 + \sum_{t=1}^T \w_t^2\|g_t\|^2}{2\cdot \w_{1:T}}\triangleq \lambda \|g_k\|^{-2}
    \end{align*}
    where we have defined $\lambda =\frac{\|x_1-\cmp\|^2 + \sum_{t=1}^T \w_t^2\|g_t\|^2}{2\cdot \w_{1:T}} $, which does not depend on $k$. That is, the optimal $\w_k$ value is proportional to $\|g_k\|^{-2}$. With this expression, we have:
    \begin{align*}
        \sum_{t=1}^T \w_t^2\|g_t\|^2 &= \lambda^2 \sum_{t=1}^T \|g_t\|^{-2}\\
        \w_{1:T} &= \lambda \sum_{t=1}^T \|g_t\|^{-2}
    \end{align*}
    So, let us now solve for $\lambda$ by plugging in these values:
    \begin{align*}
        \lambda &=\frac{\|x_1-\cmp\|^2 + \sum_{t=1}^T \w_t^2\|g_t\|^2}{2\cdot \w_{1:T}} \\
        \lambda &= \frac{\|x_1-\cmp\|^2 + \lambda^2 \sum_{t=1}^T \|g_t\|^{-2}}{2\lambda \sum_{t=1}^T \|g_t\|^{-2}} \\
        \lambda &= \frac{\|x_1-\cmp\|^2}{2\lambda \sum_{t=1}^T \|g_t\|^{-2}} + \frac{\lambda}{2}\\
        \lambda &=\frac{\|x_1-\cmp\|}{\sqrt{\sum_{t=1}^T \|g_t\|^{-2}}}
    \end{align*}
    This in turn implies the claimed optimal value for $\w_k$.
\end{proof}


\section{Proof of Theorem~\ref{thm:represent}}\label{sec:proof:represent}

\thmrepresent*

\begin{proof}
First, observe that for any solution to the desired identity $\eta_t = \frac{\w_t \w_{t:1:T}}{\w_{1:T}}$,  replacing $w$ with $c\cdot  w$ for some constant $c$ will yield a solution for $\eta$ replaced with $c\cdot \eta$. Thus, it suffices to consider the possibility that $\max_t \eta_t =1$.

The intuition for the rest of the proof is the following: Given the value for $\w_1$, we can solve for $\w_{2:T}$ using the equation $\frac{\w_t \w_{2:T}}{\w_1 + \w_{2:T}} = \eta_1$. This in turn provides us with the value of $\w_{1:T}$. Now, given $\w_{k:T}$ for any $k$ we can solve for $\w_{k}$ using the equation $\eta_k = \frac{\w_k \w_{k+1:T}}{\w_{1:T}} = \frac{\w_k (\w_{k:T} - \w_k)}{\w_{1:T}}$. Thus we may recursively compute all  the values of $w$. Each of these steps requires solving a quadratic equation.  We simply choose an initial $\w_1$ so as to ensure that all the following quadratic equations have non-negative real roots.


Specifically, set $\w_1 = \frac{2^{2T} + \sqrt{2^{4T} - 4\eta_1}}{2}$ and define $s_1=2^{2T}$. Then, recursively define for $t=2,\dots,T-1$:
\begin{align*}
    s_{t} &= s_{t-1} - \w_{t-1}\\
    \w_t &= \frac{s_t - \sqrt{s_t^2 - 4 s_1 \eta_t}}{2}
\end{align*}
and set $\w_T=s_T= s_{T-1}-\w_{T-1}$. Notice that these choices satisfy:
\begin{align*}
    \w_t^2 - s_t\w_t +s_1 \eta_t=0
\end{align*}
so that if we could establish (1) that all $\w_t\ge 0$  and (2) $s_t = \w_{t:T}$, then we would have:
\begin{align*}
    \frac{\w_t \w_{t+1:T}}{\w_{1:T}} &= \frac{\w_t (\w_{t:T} - \w_t)}{\w_{1:T}}\\
    &=\frac{\w_t (s_t -\w_t)}{s_1}\\
    &=\frac{s_t \w_t-\w_t^2}{s_1}\\
    &=\eta_t
\end{align*}
as desired. 

Let us first prove (1): all $\w_t\ge 0$. For $t\le T-1$, this will  hold if $s_t^2 - 4s_1\eta_t>0$ . To establish this, we will first show that $s_t \ge \frac{s_1}{2^{t-1}}$ for all $t\le T-1$. If this holds, then we have:
\begin{align*}
    s_t^2 \ge \frac{s_1^2}{2^{2t-2}}\ge \frac{s_1 2^{2T}}{2^{2t-2}}\ge 4s_1\ge 4s_1\eta_t
\end{align*}
for $t\le T-1$
So, we establish $s_t \ge \frac{s_1}{2^{t-1}}$ by induction for $t\le T-1$. The statement is clear for $t=1$. Suppose it holds for for all $t\le k$ for some $k\le T-2$. Then we have:
\begin{align*}
    s_{k+1} &= s_k - \w_k\\
    &= \frac{s_k + \sqrt{s_k^2 - 4s_k\eta_k}}{2}\\
    &\ge \frac{s_k}{2}\\
    &\ge \frac{s_1}{2^{k-1+1}}
\end{align*}
which establishes the claim. Therefore for $t\le T-1$, $\w_t$ are non-negative real numbers. Finally, we have:
\begin{align*}
    \w_{T-1}  &= \frac{s_{T-1}+ \sqrt{s_{T-1}^2 - 4 s_1 \eta_t}}{2}\le s_{T-1}
\end{align*}
so that $\w_T=s_T = s_{T-1}-\w_{T-1}\ge 0$. Thus $\w_t\ge 0$ for all $t$.

Next, to show (2): $s_t = \w_{t:T}$. This is nearly immediate. By definition we have $\w_T=s_T$. Suppose $s_k = \w_{t:T}$ for some $t\ge 2$. Then $s_t= s_{t-1}-\w_{t-1}$ so that $s_{t-1}=s_t+\w_{t-1}=\w_{t-1:T}$. Thus by induction we have $s_t = \w_{t:T}$ for all $t$, which is the last thing we needed to show.
\end{proof}
